Document Haystacks: Vision-Language Reasoning Over Piles of 1000+ Documents

Large multimodal models (LMMs) have achieved impressive progress in vision-language understanding, yet they face limitations in real-world applications requiring complex reasoning over a large number of images. Existing benchmarks for multi-image question-answering are limited in scope, each question is paired with only up to 30 images, which does not fully capture the demands of large-scale retrieval tasks encountered in the real-world usages. To reduce these gaps, we introduce two document haystack benchmarks, dubbed DocHaystack and InfoHaystack, designed to evaluate LMM performance on large-scale visual document retrieval and understanding. Additionally, we propose V-RAG, a novel, vision-centric retrieval-augmented generation (RAG) framework that leverages a suite of multimodal vision encoders, each optimized for specific strengths, and a dedicated question-document relevance module. V-RAG sets a new standard, with a 9% and 11% improvement in Recall@1 on the challenging DocHaystack-1000 and InfoHaystack-1000 benchmarks, respectively, compared to the previous best baseline models. Additionally, integrating V-RAG with LMMs enables them to efficiently operate across thousands of images, yielding significant improvements on our DocHaystack and InfoHaystack benchmarks. Our code and datasets are available at https://github.com/Vision-CAIR/dochaystacks

==> table/ablation_topk.tex <==
% \begin{table}
% \centering
% \resizebox{1.0 \linewidth}{!}{
%     \begin{tabular}{ccccccc}
%     \toprule
%     \multirow{2}{*}{Model} & \multicolumn{3}{c}{DocHaystack} & \multicolumn{3}{c}{InfoHaystack}  \\
%     ~ & 100 & 200 & 1000 & 100 & 200 & 1000 \\
%     \midrule
%     \multicolumn{7}{c}{w/ V-RAG top 1 retrieval}\\
%     \midrule
%     Gemini     & 62.39 & 59.63 & 39.45 & 50.32 & 48.39 & 41.94 \\
%     GPT-4o   & \textbf{67.89} & 62.39 & \textbf{44.95} & 44.52 & 46.45 & 40.00 \\
%     LLaVA-OV  & 50.46 & 45.87 & 34.86 & 34.19 & 31.61 & 26.45 \\
%     Qwen2-VL & 63.30 & 61.47 & 39.45 & 49.03 & \textbf{50.32} & \textbf{43.23} \\
%     % Qwen2-VL f.t     & 66.97 & 62.39 & 42.20 & 49.68 & 47.10 & 40.65 \\
%     % Qwen2-VL random f.t  & 66.06 & 64.22 & 44.95 & 49.68 & 49.68 & 40.00 \\
%     % Qwen2-VL f.t r32  & ~ & ~ & ~ & 47 & 45 & 36\\

%     % Qwe2-VL f.t (2 epochs)  & 64.22 & 63.30 & 42.20 & 52.9& 50.32& 43.87\\
%     Qwen2-ft-final    & 66.79 & \textbf{64.22} & 42.20 & \textbf{50.97} &  49.68  & 41.94\\
%     \midrule
%     \multicolumn{7}{c}{w/ V-RAG top 3 retrievals} \\
%     \midrule
%     Gemini   & 50.46 & 54.13 & 44.04 & 31.61 & 32.90 & 28.39 \\
%     GPT-4o  & 75.23 & 76.15 & 65.14 & 56.77 & 54.84 & 49.03 \\
%     LLaVA-OV & 58.73 & 55.96 & 49.54 & 30.97 & 34.84 & 25.81 \\
%     Qwen2-VL  & 72.48 & 72.48 & 59.63 & 55.48 & 58.71 & 49.03 \\
%     % Qwen2-VL f.t      & 77.98 & 75.23& 63.30 & 53.55 & 56.77 & 49.68 \\
%     % Qwen2-VL random f.t  & 78.90 & 77.06 & 63.30 & 56.13 & 55.48 & 47.74 \\
%     % % Qwen2-VL f.t (all data)     & ~ & ~ & ~ & 55.48 & 54.19 & 43.87\\
%     % % Qwen2-VL random f.t  & ~ & ~ & ~ & 52.90 & 54.84 & 45.16 \\
%     % Qwen2-VL f.t r32  & ~ & ~ & ~ & 54 & 53 & 47\\
%     % Qwe2-VL f.t (2 epochs)  & 77.06 & 74.31 & 65.14 & 56.13& 60.65& 50.32\\
%     Qwen2-ft-final    & \textbf{77.98} & \textbf{77.06} & \textbf{ 65.14} & \textbf{58.06} & \textbf{59.35} & \textbf{50.32}\\

%     % \midrule
%     % \multicolumn{7}{c}{Top 4 retrievals} \\
%     % \midrule
%     % LLaVA-OV + V-RAG & 57.80 & 50.46 & 44.95 & 29.68 & 28.39 & 27.74 \\
%     \midrule
%     \multicolumn{7}{c}{w/ V-RAG top 5 retrievals} \\
%     \midrule
%     Gemini  & 55.96 & 53.21 & 53.21 & 34.19 & 36.77 & 31.61 \\
%     GPT-4o   & 72.48 & \textbf{78.90} & 67.89 & 52.90 & 56.13 & 49.68 \\
%     LLaVA-OV  & 28.44 & 22.02 & 20.18 & 16.13 & 18.06 & 13.55 \\
%     Qwen2-VL & 75.23 & 70.64 & 66.06 & 58.71 & 57.42 & 54.84 \\
%     % Qwen2-VL f.t    & 77.06 & 77.98 & 72.48 & 61.94 & 57.42 & 50.32 \\
%     % Qwen2-VL random f.t & 77.98 & 77.98 & 67.89 & 60.00 & 56.13 & 49.68\\
%     % Qwen2-VL f.t r32  & ~ & ~ & ~ & 61 & 54 & 47\\
%     % Qwe2-VL f.t (2 epochs)  & 76.15 &  74.31 & 70.64 & 62.58& 58.06& 52.90\\
%     Qwen2-ft-final    & \textbf{78.90} & 77.98 & \textbf{68.81} & \textbf{62.58} & \textbf{58.71} & \textbf{54.84}\\
%     \bottomrule
%     \end{tabular}
% }
% \caption{\textbf{Ablation study on the impact of the number of top-k retrieved images.} We evaluate how different values of top-k affect final visual question answering accuracy on the DocHaystack and InfoHaystack benchmarks.}
% \label{tab:topk}
% \end{table}
